Deep 6-DOF Tracking

We present a temporal 6-DOF tracking method which leverages deep learning to achieve state-of-the-art performance on challenging datasets of real world capture. Our method is both more accurate and more robust to occlusions than the existing best performing approaches while maintaining real-time performance. To assess its efficacy, we evaluate our approach on several challenging RGBD sequences of real objects in a variety of conditions. Notably, we systematically evaluate robustness to occlusions through a series of sequences where the object to be tracked is increasingly occluded. Finally, our approach is purely data-driven and does not require any hand-designed features: robust tracking is automatically learned from data.

==> Sections/Overview.tex <==
%!TEX root = ../main.tex
\section{Tracking with deep learning} 

Temporal tracking is different than ``tracking by detection'' in that the temporal tracker uses two frames adjacent in time, and assumes knowledge of the object pose at the previous frame. To train a deep network on that task, one could straightforwardly used the current and previous RGBD frames directly as input. Unfortunately, while doing so yields low prediction errors on a ``conventional'' machine learning test set (composed of pairs of frames as input and rigid pose as target), it completely fails in the closed loop scenario. Indeed, since the network never learned to correct itself, small errors accumulate rapidly and tracking is lost in a matter of milliseconds. Another solution could be to provide the previous estimate of the pose change instead of the previous RGBD frame as input to the network. In this case, this information alone is not rich enough to enable the network to learn robust high level representations, so tracking errors are very high. 

To solve this problem, we propose to use an \emph{estimate} of the object pose from the previous timestep in the sequence as input to the network, in addition to the current RGBD frame. This allows the network to correct errors made in closed loop tracking. The estimate of the current object pose is obtained by rendering a synthetic RGBD frame of the tracked object. 

In the remainder of the paper, we first describe how training data is generated in~\autoref{sec:data-generation}, and the proposed CNN architecture and learning methodology in~\autoref{sec:learning}. An extensive series of experiments evaluating our approach against the state-of-the-art method of Tan et al.~\cite{tan-iccv-15} on a varied real dataset with ground truth is presented in~\autoref{sec:experiments}. Our approach is more stable, yields lower errors, and is more robust to occlusion that \cite{tan-iccv-15} in all the scenarios we tested. 

